Improving Log-Cumulant Based Estimation of Roughness Information in SAR imagery

Synthetic Aperture Radar (SAR) image understanding is crucial in remote sensing applications, but it is hindered by its intrinsic noise contamination, called speckle. Sophisticated statistical models, such as the $\mathcal{G}^0$ family of distributions, have been employed to SAR data and many of the current advancements in processing this imagery have been accomplished through extracting information from these models. In this paper, we propose improvements to parameter estimation in $\mathcal{G}^0$ distributions using the Method of Log-Cumulants. First, using Bayesian modeling, we construct that regularly produce reliable roughness estimates under both $\mathcal{G}^0_A$ and $\mathcal{G}^0_I$ models. Second, we make use of an approximation of the Trigamma function to compute the estimated roughness in constant time, making it considerably faster than the existing method for this task. Finally, we show how we can use this method to achieve fast and reliable SAR image understanding based on roughness information.

==> Fast_approach.tex <==
\section{Fast approach for log-cumulants method} \label{sec:fast}

In this section we present a fast approach for log-cumulants method to estimate the parameters $(\alpha, \gamma)$ of the $G_I^0$ distribution. For solving the systems of non-linear equations in (\ref{EqSistLogCumgi0}), we used the follow identity \cite{REF_book_Arfken}:

\begin{equation}\label{identidade_1}
	{\Psi^n(w)} = \frac{d^{n+1}\textrm{ln}(\Gamma(w))}{dw^{n+1}},
\end{equation}

\noindent where $n \in\mathbb{N^*}$ and $w >0$. Another important identity for this paper is \cite{REF_book_Abramowitz}: 

\begin{equation}\label{identidade_2}
	{\Gamma(w)} = \frac{1}{we^{{\tau}w}{\prod_{k=1}^{\infty}}\left(1+\frac{w}{k}\right)e^{-\frac{w}{k}}},
\end{equation}

\noindent where $\tau$ is the Euler-Macheroni constant.

Applying the natural logarithm in (\ref{identidade_2}), obtain that:

\begin{equation}\label{identidade_3}
	\textrm{ln}({\Gamma(w)}) = -\textrm{ln}(w)-{\tau}w-\sum_{k=1}^{\infty}\left[\textrm{ln}\left(1+\frac{w}{k}\right)-\frac{w}{k}\right].
\end{equation}

Here, we used (\ref{identidade_1}) and (\ref{identidade_3}) to rewrite the term $\Psi^1(-\alpha)$ in the systems of non-linear equations in (\ref{EqSistLogCumgi0}) as:

\begin{equation}\label{identidade_4}
	{\Psi^1(-\alpha)} = \frac{d^{2}\textrm{ln}(\Gamma(-\alpha))}{d(-\alpha)^{2}}.
\end{equation}

\noindent Developing the partial derivatives in the right side  in (\ref{identidade_4}), were $\textrm{ln}({\Gamma(-\alpha)})$ is given by (\ref{identidade_3}), we have:

\begin{equation}\label{identidade_5}
	{\Psi^1(-\alpha)} = \frac{1}{(-\alpha)^2}+\sum_{k=1}^{\infty}\frac{1}{(k-\alpha)^2}.
\end{equation}

\noindent The magnitude order of term $\sum_{k=1}^{\infty}\frac{1}{(k-\alpha)^2}$ not exceeding of $\frac{1}{-\alpha}$. Here, this fact is denoted by \cite{REF_book_khuri}:

\begin{equation}\label{identidade_6}
	\sum_{k=1}^{\infty}\frac{1}{(k-\alpha)^2} = O\left(\frac{1}{-\alpha}\right).
\end{equation}

Our proposed is used the first term of infinite sum in (\ref{identidade_5}) as an approximation to $\Psi^1(-\alpha)$, i.e.,

\begin{equation}\label{identidade_7}
	{\Psi^1(-\alpha)} = \frac{1}{\alpha^2} + O\left(\frac{1}{-\alpha}\right),
\end{equation}

\noindent $\forall$ $\alpha<0$. Here, is important to emphasize that the term not considered in the approximation proposed will have less impact when alpha decreases, i.e., $\alpha \rightarrow -\infty$. Fig. \ref{fig_approx} shows this behavior. 

\begin{figure}[h!]
\centering
	\includegraphics[width= 0.6\linewidth]{images/approx.pdf}
	 \caption{$\Psi^1(-\alpha)$ and $\frac{1}{\alpha^2}$}
     \label{fig_approx}
\end{figure}

Using the approximation proposed and replacing in the second equation in \ref{EqSistLogCumgi0}, we have the estimator for texture parameter:

\begin{equation}\label{identidade_8}
\widehat{\alpha}=
\left \{
\begin{array}{cc}
-\left| \sqrt{\frac{1}{\widetilde{k}_2-\Psi^1(L)}} \right|, & \widetilde{k}_2-\Psi^1(L) < 0 \\\\
-\sqrt{\frac{1}{\widetilde{k}_2-\Psi^1(L)}} , & \widetilde{k}_2-\Psi^1(L) > 0. \\
\end{array}
\right.
\end{equation}

\noindent For the cases that $\Psi^1(L)-\widetilde{k}_2 =0$, is not possible to estimate the texture parameter. However, this cases are rare. The estimate of the scale parameter is obtained puting $\widehat{\alpha}$ in the first equation in (\ref{EqSistLogCumgi0}). Thus, the parameter $\gamma$ is obtained by:

\begin{equation}\label{identidade_9}
	\widehat{\gamma}=\textrm{exp}{\left[\widetilde{k}_1-\Psi^0(L)+\Psi^0(-\widehat{\alpha})\right]L}.
\end{equation}

Here, we called this estimation method of Fast Method of Log-Cumulants (FMoLC).

Alixandre a estrutura para indicar e comentar  o limite superior de sua aproximação me pareceu casar com a ideia deste trecho para vc usar o que dele for útil, principalmente em red.

As examples we give tables for FMT (u) for a number of Gaussian processes. When the length of the interval T increases, one needs an increasing number of terms in the Rice series so as not {\color{red} to surpass a given bound for the error.}  



==> Log-cumulant.tex <==
\section{The log-cumulants method} \label{sec:Log_cum_met}

Let $Z$ be a continuous random variable with probability density function $f_Z (z,\theta)$ defined over $\mathbb{R}^+$, where $\theta$ can be either a real-valued
parameter or a vector. The construction of the MoLC is based on the Mellin transform of $f_Z (z,\theta)$, which is defined by:  
\begin{equation}\label{mellin}
\phi_Z(s)=\int^\infty_0 u^{s-1}f_Z(u,\theta)\mathrm{d}u = E[Z^{s-1}].
\end{equation}

There are two important relations for the construction of the MoLC: log-moment and log-cumulant of order $v$. Is possible to obtain analytical expressions for the log-moment and log-cumulant of order $v$ by simple derivation, evaluated at $s = 1$. The log-moment of order $v$ is obtained by \cite{REF_Nicolas}:
\begin{equation}\label{logmom}
	\widetilde{m}_v = \frac{\mathrm{d}^v\phi_z(s)}{\mathrm{d}s^v}\bigg|_{s=1}, \, v\in\mathbb{N}^*.
\end{equation} 

Based on the natural logarithm of $\phi_Z(s)$, can be obtained the log- cumulant of order $v$ by    \cite{REF_Nicolas}:

\begin{equation}\label{logcum}
	\widetilde{k}_v = \frac{\mathrm{d}^v\psi_z(s)}{\mathrm{d}s^v}\bigg|_{s=1}, \, v\in\mathbb{N}^*,
\end{equation}

\noindent with $\psi_z(s)$ $=$ $log((\phi_z(s))$. 

The strategy of the MoLC to estimate $\theta$ is based on the relation between log-moment and log-cumulant. The log-cumulants can be retrieved from the
log-moments by the relation:
\begin{equation}\label{rel_logMom}
        \widetilde{k}_v= \widetilde{m}_v - \sum_{i=1}^{v-1}\left( \begin{array}{c}
{r-1} \\
{i-1} \end{array} \right) \widetilde{k}_i \widetilde{m}_{v-i}.
	\end{equation}

\noindent For example, the log-cumulants and log-moments of order 1 and 2 are related by:
	\begin{numcases}\\
	\widetilde{k}_1 = \widetilde{m}_1\label{EqLogCum1} \nonumber \\
	\hspace{3cm}\\
    \widetilde{k}_2 = \widetilde{m}_2 - \widetilde{m}_1^2.\label{EqLogCum2}\nonumber
	\end{numcases}


Usually, to estimate the parameter $\Theta$ replaced $\widetilde{m}_v$ by the corresponding sample log-moment, which is given by \cite{REF_Nicolas}: 
	
\begin{equation}\label{logMomEstim}
        \widehat{\widetilde{m}}_v = \frac{1}{n}\sum_{i=1}^n\log z_i^v,
	\end{equation}
  
\noindent with $z_i$, $i\in\ \{1, 2,..., n\}$, being a sample of a random variable $Z$.

In the next section, we present the construction of the MoLC to estimate the parameters of the probability density functions proposed by \emph{Frery et al.} \cite{REF_Frery}, known as $G_I^0$ distribution.


\section{The log-cumulants method for the $G_I^0$ distribution} \label{sec:Log-cum_gi0}

The $G_I^0$ continuous distribution, with parameter vector $\theta=(\alpha, \gamma, L)$, is characterized by the following probability density function \cite{REF_Frery}:
\setlength{\arraycolsep}{0.0em}
	\begin{eqnarray}\label{gi0}
	f_{G_I^0}(z,\theta )&{}={}& \frac{L^{L}\Gamma(L-\alpha)}{\gamma^{\alpha}\Gamma(-\alpha)\Gamma(L)} z^{L-1}(\gamma+Lz)^{\alpha - L},
	\end{eqnarray}
	\setlength{\arraycolsep}{5pt} 

\noindent where $z>0$, $\alpha <0$ is the texture parameter, $\gamma>0$ the scale parameter, $L \geq 1$ number of looks and $\Gamma(.)$ the gamma function. The corresponding $r$th-order moment for the $G_I^0$ distribution is given by:

\begin{equation}\label{Eq_EGi0}
 E_{G_I^0}[Z^r]=
		\left( \frac{\gamma}{L}\right)^r \frac{\Gamma(-\alpha-r)\Gamma(L+r)}{\Gamma(-\alpha)\Gamma(L)},
	\end{equation}
    
\noindent with $\alpha<-r$.

For the probability density function in (\ref{gi0}) the function $\phi_Z(s)$ can be obtain using (\ref{mellin}). For this, we used (\ref{Eq_EGi0}) replaced $E[Z^{s-1}]$ the $G_I^0$ distribution is given by:
\begin{equation}\label{phi_gi0}
{\phi_{G_I^0}(s)=}
		\left( \frac{\gamma_I}{L_I}\right)^{s-1} \frac{\Gamma(1-s-\alpha_I)\Gamma(L_I+s-1)}{\Gamma(-\alpha_I)\Gamma(L_I)}.
	\end{equation}
    
In this paper we assumed the parameter $L$  known. Thus, using (\ref{logcum}) we have the log-cumulants of order 1 and 2 for $G_I^0$ distribution:
\setlength{\arraycolsep}{0.0em}
	\begin{numcases}\\ 
	\widetilde{k}_1 = \log \left(\frac{\gamma}{L} \right) +\Psi^0(L)-\Psi^0(-\alpha)\label{EqSistLogCum1} \nonumber \\
	\widetilde{k}_2 = \Psi^{1}(L) +\Psi^{1}(-\alpha) \label{EqSistLogCumgi0},
	\end{numcases}
	\setlength{\arraycolsep}{5pt}

\noindent where $\Psi^0(.)$ and $\Psi^1(.)$ are the digamma and trigamma function, respectively.

To estimate the parameters vectors $\theta^*=(\alpha, \gamma)$, we used the equations (\ref{EqSistLogCum1}) and the relation (\ref{EqLogCum1}) replacing $\widetilde{m}_1$ and $\widetilde{m}_2$ by the corresponding sample log-moments, given by (\ref{logMomEstim}).

Given that there are not inverse functions for $\Psi^0(.)$ and $\Psi^1(.)$, the solutions of the non-linear systems (\ref{EqSistLogCum1}) cannot be obtained explicitly and iterative procedures are needed. Generally this procedures are computationally slow, and reduce the computational cost is an important challenge.



==> cover_letter/preamble.tex <==
\usepackage{mdframed} % Add easy frames to paragraphs
\usepackage{lipsum} % For dummy text
\usepackage{xcolor}
\usepackage{enumerate}
\usepackage{booktabs}
\usepackage{xparse} 
\usepackage[english]{babel}
\usepackage{lscape}
\usepackage{array}
\usepackage[margin=0.9in]{geometry}
% Add support for \NewDocumentEnvironment
\definecolor{graylight}{rgb}{0,0,0} % define color using xcolor syntax

\usepackage[explicit]{titlesec}
\usepackage{xhfill}




%\titleformat{\section}[block]{\LARGE\bfseries\filcenter}{#1}{1em}{}
\titleformat{\section}[display]{\bfseries\Large}{}{1em}{#1}
\titleformat{\subsection}[display]{\bfseries\large}{}{1em}{#1\space\xrfill[0.6ex]{0.4pt}}

\newmdenv[ % Define mdframe settings and store as leftrule
  linecolor=graylight,
  topline=false,
  bottomline=false,
  rightline=false,
  skipabove=\topsep,
  skipbelow=\topsep
]{leftrule}

\NewDocumentEnvironment{response}{O{\textbf{Response:}}} % Define example environment
{\begin{leftrule}\small \noindent\textcolor{graylight}{#1}\par}
{\end{leftrule}}

\newcolumntype{L}[1]{>{\RaggedRight\arraybackslash}p{#1}}

